Symmetry-Based Singlet-Triplet Excitation in Solution Nuclear Magnetic Resonance

Coupled pairs of spin-1/2 nuclei support one singlet state and three triplet states. In many circumstances the nuclear singlet order, defined as the difference between the singlet population and the mean of the triplet populations, is a long-lived state which persists for a relatively long time in solution. Various methods have been proposed for generating singlet order, starting from nuclear magnetization. This requires the stimulation of singlet-to-triplet transitions by modulated radiofrequency fields. We show that a recently described pulse sequence, known as PulsePol (Schwartz $\textit{et al.}$, Science Advances, $\textbf{4}$, eaat8978 (2018) and arXiv:1710.01508), is an efficient technique for converting magnetization into long-lived singlet order. We show that the operation of this pulse sequence may be understood by adapting the theory of symmetry-based recoupling sequences in magic-angle-spinning solid-state NMR. The concept of riffling allows PulsePol to be interpreted using the theory of symmetry-based pulse sequences, and explains its robustness. This theory is used to derive a range of new pulse sequences for performing singlet-triplet excitation and conversion in solution NMR. Schemes for further enhancing the robustness of the transformations are demonstrated.

==> Figures/tauRdependence.tex <==
\begin{figure}[tb]
\centering
%\includegraphics[width=0.95\columnwidth]{Graphics/TauVarV5.png}
\includegraphics[width=0.95\columnwidth]{Graphics/tau_mismatch.pdf}
\caption{\label{fig:sequence} Experimental $^{13}{\rm C}$ signal amplitudes (white dots) for (a) \Rsymm431, (b) \Rsymm873 and (c) M2S as a function of the relative inter-pulse delay mismatch $\Delta \tau/\tau^{0}$, where $\tau^{0}$ represents the nominal inter-pulse delay. For the M2S sequence the nominal inter-pulse delay is given by $\tau^{0}=1/(4 J)$, whereas for R-based sequences the nominal inter-pulse delay is given by $\tau^{0}=n/(N J)$. The R-sequences have been implemented according to the PulsePol procedure summarised in figure~\ref{fig:Rseqstandard}. The final $^{13}{\rm C}$ signal amplitudes were referenced with respect to a single $^{13}{\rm C}$-pulse-acquire spectrum. Light blue trajectories represent numerical simulations with the pulse sequence parameters given in table~\ref{tab:SOExcPars}. Relaxation was neglected in all cases.%\NWnote{just out of curiosity: Is the difference to theory just relaxation/imperfect pulses? The profiles in a and b are slightly asymmetric, is this because the total sequence length is different for different $\tau$ values? somehow I would have expected it to be skewed the other way then, or am I reading the $x$-axis the wrong way? (I interpret it as: on the left, $\tau$ is shorter.)}
%\MHLnote{Most of the caption will be discarded. Horizontal scale must have tick marks at conventional positions such as 12.0, 13.0, etc. }
}
\end{figure}

==> Tables/SOExcPars.tex <==
 \begin{table}[tb]
 \renewcommand{\arraystretch}{1.5}
  \begin{tabular*}{0.4\textwidth}{@{\extracolsep{\fill}}lll}
\hline
    $\omega_{nut}/(2\pi)$ & $12.5$ kHz
\\
    $\tau_{90}$ & 20 $\mu$s
\\
\hline
\multirow{4}{4em}{\Rsymm431 (PulsePol)}
 &   $\tau_R$    & 13800 ${\,\mu \mathrm{s}}$
\\
 &   $\tau$    & 6860 ${\,\mu \mathrm{s}}$
\\
 &   $n_R^\mathrm{exc}$       &  9
\\
 &   $\tau_\mathrm{exc}$     & 124.2 ms
 \\ \hline
 \multirow{4}{4em}{\Rsymm431 (standard)}
 &   $\tau_R$    & 13400 ${\,\mu \mathrm{s}}$
\\
 &   $\tau$    & 6660 ${\,\mu \mathrm{s}}$
\\
 &   $n_R^\mathrm{exc}$       &  9
\\
 &   $\tau_\mathrm{exc}$     & 120.60 ms
\\ \hline
\multirow{4}{4em}{\Rsymm873 (PulsePol)} 
 &   $\tau_R$    & 16000 ${\,\mu \mathrm{s}}$
\\
 &   $\tau$    & 7960 ${\,\mu \mathrm{s}}$
\\
 &   $n_R^\mathrm{exc}$       &  9
\\
 &   $\tau_\mathrm{exc}$     & 144.00 ms
  \\ \hline
 \multirow{4}{4em}{\Rsymm873 (standard)}
 &   $\tau_R$    & 15560 ${\,\mu \mathrm{s}}$
\\
 &   $\tau$    & 7740 ${\,\mu \mathrm{s}}$
\\
 &   $n_R^\mathrm{exc}$       &  9
\\
 &   $\tau_\mathrm{exc}$     & 140.04 ms
\\ \hline
\multirow{4}{4em}{\Rsymm{10}32} 
 &   $\tau_R$    & 5560 ${\,\mu \mathrm{s}}$
\\
 &   $\tau$    & 2720 ${\,\mu \mathrm{s}}$
\\
 &   $n_R^\mathrm{exc}$       &  38
\\
 &   $\tau_\mathrm{exc}$     & 211.30 ms
\\ \hline
\multirow{4}{4em}{M2S} 
 &   $\tau_\mathrm{echo}$    & 9240 ${\,\mu \mathrm{s}}$
\\
 &   $\tau_1$    & 4580 ${\,\mu \mathrm{s}}$
 \\
 &   $\tau_2$    & 4600 ${\,\mu \mathrm{s}}$
\\
 &   $n_1$       &  11
\\
 &   $n_2$       & 5
 \\
 &   $\tau_\mathrm{exc}$     & 152.46 ms
\\ \hline
  \end{tabular*}
 \caption{
 \label{tab:SOExcPars}
 Experimental parameters for the \RNnnu sequences used to obtain the results in figure~\ref{fig:SingletFilteredSpectra}(c,d,e,f). The parameters have
 the same meaning as in table~\ref{tab:OuterSTexcPars}. The parameters are given separately for \Rsymm431 sequences (used in figure~\ref{fig:SingletFilteredSpectra}(c,e)), and for \Rsymm873 sequences (used in figure~\ref{fig:SingletFilteredSpectra}(d,f)). M2S is the sequence $90_{x}-(\tau_{1}-90_{y}180_{x}90_{y}-\tau_{1})^{n_1}-90_{y}-\tau_{2}-(\tau_{1}-90_{y}180_{x}90_{y}-\tau_{1})^{n_2}$. Where the individual spin echoes have total duration $\tau_\mathrm{echo}$, and $n_1$ and $n_2$ denote the number of repetitions. Taking into account the finite duration of the pulses, $\tau_1$ is the interval \emph{between} pulses in the spin echoes, and $\tau_2$ is the interval after the $90_{y}$ pulse. The echoes are implemented with the standard MLEV-4 four-step [0,0,180,180] supercycle~\cite{levitt_broadband_1982,pileio_storage_2010,tayler_theory_2012}.   
 \MHLnote{Table to be moved to SI}
 } 
\end{table}
